Dataless Knowledge Fusion by Merging Weights of Language Models

Fine-tuning pre-trained language models has become the prevalent paradigm for building downstream NLP models. Oftentimes fine-tuned models are readily available but their training data is not, due to data privacy or intellectual property concerns. This creates a barrier to fusing knowledge across individual models to yield a better single model. In this paper, we study the problem of merging individual models built on different training data sets to obtain a single model that performs well both across all data set domains and can generalize on out-of-domain data. We propose a dataless knowledge fusion method that merges models in their parameter space, guided by weights that minimize prediction differences between the merged model and the individual models. Over a battery of evaluation settings, we show that the proposed method significantly outperforms baselines such as Fisher-weighted averaging or model ensembling. Further, we find that our method is a promising alternative to multi-task learning that can preserve or sometimes improve over the individual models without access to the training data. Finally, model merging is more efficient than training a multi-task model, thus making it applicable to a wider set of scenarios.

==> iclr2023/chaps/abs-old.tex <==
\begin{abstract}
% The prevalent application of language model fine-tuning has produced numerous fine-tuned models with different skills. Combining knowledge of these models, \textit{e.g.} two domain-specific named entity recognition models from a public model repository, however, is non-trivial. A common practice is to retrain a new model over joint training sets, which is inefficient and can be infeasible due to data privacy. In this paper, we address the challenge by merging models directly in the weight space. The goal of model merging is to obtain a single model (of the same architecture and size) that solves all domains or tasks; furthermore, by fusing knowledge of individual models, we expect to achieve decent generalization over domains unseen by any individual models. %Unfortunately, experiments show that simply averaging the weights performs poorly. 
% The main technical challenge is the algorithm for merging the models.
% We propose a novel algorithm, \method{}, inspired by the optimal merged weights that minimize $\ell^2$ distances between the outputs of the merged and individual models in linear models.
% %which obtains merged model weights by solving a linear regression problem for each layer in transformer-based language models with low dimensional input statistics. 
% The algorithm provides a closed-form solution, is extendable to merging any number of models, while significantly outperforms other model merging baselines, such as simple weight averaging. We perform extensive evaluation and analysis in various levels of difficulties to facilitate future research.

% Language model fine-tuning using supervised data is the prevalent paradigm for solving many NLP tasks and combining data from multiple related data sets, domains or tasks is usually beneficial. 
Fine-tuning pre-trained language models has become the prevalent paradigm for building models for downstream NLP tasks such as classification or sequence tagging. Oftentimes fine-tuned models are readily available but their training data is not due to data privacy or intellectual property concerns. This creates a barrier to fusing knowledge across multiple models to yield a better \textit{multi-task} model.
% However, this annotated data may not always be available for fine-tuning models due to privacy or IP concerns, despite models being publicly shared by individuals or organizations. 
In this paper, we aim to address this unique challenge by merging models in the weight space with the goal of obtaining a single model that can perform well on the domains it was trained on and have the ability to generalize. We propose a novel method inspired by the optimal merged weights that minimize $\ell^2$ distances between the outputs of the merged and individual linear models. We introduce a battery of testing setups for the model merging task including training over different label distributions and domains. Our results show that our proposed approach significantly outperforms alternatives such as simple weight averaging. Further, we see that our method for model merging is a promising alternative to multi-task learning and improves performance over individual models in specific setups, while being faster and more efficient, making it applicable to a wider set of scenarios.
\end{abstract}

==> iclr2023/maintabs/emotion_merge_all.tex <==
\begin{table}[]
\centering
\scalebox{0.76}{
\begin{tabular}{@{}lcacacacacaca@{}}
\toprule
\rowcolor{white}  &    \multicolumn{2}{c}{Avg. $f_{1..k}$}        & \multicolumn{2}{c}{Best $f_{1..k}$} & \multicolumn{2}{c}{Simple} & \multicolumn{2}{c}{Fisher} & \multicolumn{2}{c}{RegMean} & \multicolumn{2}{c}{Multi-Task} \\  \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(l){10-11}  \cmidrule(l){12-13} 
%\multicolumn{13}{c}{\textbf{Emotion}} \\ \midrule
 & ID & OOD & ID & OOD  & ID & OOD & ID & OOD  & ID & OOD & ID & OOD \\ 
 
\cmidrule(r){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(l){10-11}  \cmidrule(l){12-13} 

\rowcolor{white}  RoBERTa-base  &       & &    &       &    &       &     &  &        &     &        &      \\
- \textit{w/ Same Head Init.}  &    18.91   & 21.71  &  23.98   &   31.94              & 20.92         & 11.17         & 26.52       &  20.67         & 38.73         & 22.75        &  47.75            & 28.29          \\
- \textit{w/ Diff Head Init.}   &   18.91    & 21.71 &    23.98     &    31.94           &    0.00       &    0.00      &    23.59  &  18.76    &   32.44   &    15.53     &     47.75     &    28.29     \\
T5-base   &   -    &  30.30  &  -             & 38.85              &  -         & 38.77         & -       & 37.84        & -         &    39.58        & -            & -           \\
%DeBERTa-Large   &       &    & 100               & 100              & 100          & 100         & 100          & 100         & 100          & 100          & 100            & 100           \\ \midrule
\bottomrule
\end{tabular}
}
\caption{\small{Performance over in-domain and out-of-domain test sets when merging all 5 domain-specific emotion classification models.}}
\label{tab:merge_all_emotion}
\end{table}

==> iclr2023/maintabs/emotion_roberta_diffseed_pair.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\scalebox{0.76}{
\begin{tabular}{@{}ll|cc|cc|cc|cc|cc|cc@{}}
\toprule
$D_1$         & $D_2$       & \multicolumn{2}{c}{$f_1$} & \multicolumn{2}{c}{best($f_1$,$f_2$)} & \multicolumn{2}{c}{Simple} & \multicolumn{2}{c}{Fisher} & \multicolumn{2}{c}{RegMean} & \multicolumn{2}{c}{Multi-Task} \\ 
\cmidrule(r){1-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(l){13-14}
\rowcolor{Gray} \multicolumn{14}{c}{\textbf{RoBERTa-base}} \\ \midrule
DD   & CF & 45.58       & 13.00       & 45.58       & 29.98       & 18.94        & 8.28        & 21.46        & 25.22       & 40.67        & 20.28        & 43.61          & 27.91         \\
CF   & Tec         & 29.98       & 22.69       &  29.98       & 58.90       & 12.09        & 18.95       & 23.69        & 37.15       & 26.77        & 44.10        & 26.95          & 51.69         \\
Tec           & Tales       & 58.90       & 17.65       & 58.90       & 49.10       & 8.68         & 35.31       & 57.66        & 19.83       & 48.26        & 45.74        & 57.51          & 48.63         \\
Tales         & Isear       & 49.10       & 28.32       & 49.10       & 71.33       & 33.89        & 43.25       & 23.56        & 61.61       & 45.80        & 69.56        & 48.11          & 71.69         \\
\multicolumn{14}{c}{...}           \\ \midrule
\rowcolor{white} \multicolumn{2}{l}{20 Comb. Avg.}              & \multicolumn{2}{c}{18.72} & \multicolumn{2}{c}{50.98} & \multicolumn{2}{c}{23.22}  & \multicolumn{2}{c}{33.77}  & \multicolumn{2}{c}{44.17}   & \multicolumn{2}{c}{51.71}      \\ \midrule




\rowcolor{Gray} \multicolumn{14}{c}{\textbf{T5-base}} \\ \midrule

DD     & CF     & 41.54          &          &     41.54      & 37.30         & 42.11        & 31.83       & 41.19        & 33.22       & 37.68        & 34.72        &                &               \\
CF     & Tec             & 37.30          &          &    37.30        & 55.97         & 27.65        & 50.86       & 36.73        & 31.88       & 30.81        & 48.52        &                &               \\
Tec             & Tales           & 55.97          &          &     55.97         & 45.50         & 51.73        & 29.94       & 32.96        & 42.34       & 50.97        & 36.27        &                &               \\
Tales           & Isear           & 45.50          &          &    45.50       & 70.66         & 29.52        & 69.47       & 42.52        & 46.34       & 37.82        & 69.58        &                &               \\

\multicolumn{14}{c}{...}           \\ \midrule
\rowcolor{white} \multicolumn{2}{l}{20 Comb. Avg.}              & \multicolumn{2}{c}{} & \multicolumn{2}{c}{47.96} & \multicolumn{2}{c}{41.73}  & \multicolumn{2}{c}{40.29}  & \multicolumn{2}{c}{45.57}   & \multicolumn{2}{c}{}      \\  \midrule



\rowcolor{Gray} \multicolumn{14}{c}{\textbf{DeBERTa-Large}} \\ \midrule

% DD     & CF     & 41.54          &          &     41.54      & 37.30         & 42.11        & 31.83       & 41.19        & 33.22       & 37.68        & 34.72        &                &               \\
% CF     & Tec             & 37.30          &          &    37.30        & 55.97         & 27.65        & 50.86       & 36.73        & 31.88       & 30.81        & 48.52        &                &               \\
% Tec             & Tales           & 55.97          &          &     55.97         & 45.50         & 51.73        & 29.94       & 32.96        & 42.34       & 50.97        & 36.27        &                &               \\
% Tales           & Isear           & 45.50          &          &    45.50       & 70.66         & 29.52        & 69.47       & 42.52        & 46.34       & 37.82        & 69.58        &                &               \\

%\multicolumn{14}{c}{...}           \\ \midrule
\rowcolor{white} \multicolumn{2}{l}{20 Comb. Avg.}              & \multicolumn{2}{c}{} & \multicolumn{2}{c}{49.78} & \multicolumn{2}{c}{7.72}  & \multicolumn{2}{c}{30.83}  & \multicolumn{2}{c}{37.38}   & \multicolumn{2}{c}{}      \\  




\bottomrule
\end{tabular}
}
\caption{}
\label{Pairwise}
\end{table}

% \cmidrule(r){1-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(l){13-14}

==> iclr2023/maintabs/ner_merge_all.tex <==
\begin{wraptable}{r}{0.5\textwidth}
\centering
\scalebox{0.8}{
\begin{tabular}{@{}lccc@{}}
\toprule
                 & In-domain & CoNLL & Twitter \\ \midrule
Avg. $f_{1..k}$  & 77.02     & 67.91 & 44.50   \\
Best. $f_{1..k}$ & 88.46     & 80.24 & 58.40   \\ 
MTL              & 90.42     & 78.53 & 33.21   \\ 
\midrule
Simple           & 81.63     & 73.92 & 48.07   \\
Fisher           & 76.75     & 68.68 & 45.81   \\
RegMean          & 85.68     & 78.27 & 50.70   \\ \bottomrule
\end{tabular}}
\caption{\small{\small{Performance over in-domain and out-of-domain test sets (CoNLL, Twitter) when merging all 6 domain-specific RoBERTa-base NER models.}}}
\label{tab:merge_all_ner}
\end{wraptable}
